MedKLIP: Medical Knowledge Enhanced Language-Image Pre-Training in Radiology

In this paper, we consider enhancing medical visual-language pre-training (VLP) with domain-specific knowledge, by exploiting the paired image-text reports from the radiological daily practice. In particular, we make the following contributions: First, unlike existing works that directly process the raw reports, we adopt a novel triplet extraction module to extract the medical-related information, avoiding unnecessary complexity from language grammar and enhancing the supervision signals; Second, we propose a novel triplet encoding module with entity translation by querying a knowledge base, to exploit the rich domain knowledge in medical field, and implicitly build relationships between medical entities in the language embedding space; Third, we propose to use a Transformer-based fusion model for spatially aligning the entity description with visual signals at the image patch level, enabling the ability for medical diagnosis; Fourth, we conduct thorough experiments to validate the effectiveness of our architecture, and benchmark on numerous public benchmarks, e.g., ChestX-ray14, RSNA Pneumonia, SIIM-ACR Pneumothorax, COVIDx CXR-2, COVID Rural, and EdemaSeverity. In both zero-shot and fine-tuning settings, our model has demonstrated strong performance compared with the former methods on disease classification and grounding.

==> content/03_Method_backup.tex <==
\section{Method}
In this section, we start by describing the considered problem scenario in Sec.~\ref{sec:problem_scenario}, followed by the details of our proposed approach, 
including, data pre-processing by a report filter~(Sec.~\ref{sec:preprocessing}),
knowledge-enhanced entity encoding~(Sec.~\ref{sec:knowledge}), 
and the novel Transformer-based architecture for aligning the visual and language signals.

%To leverage the medical knowledge we design three parts:
%\textbf{Report Filter}, \textbf{Knowledge Encoder}, \textbf{Transformer Decoder}. In the following, we will first introduce the main framework of our method. Then we will talk about these modules one by one and discuss the intuition motivating us.

\subsection{Problem Scenario}
\label{sec:problem_scenario}

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{latex/figure/network.pdf}
    \caption{The whole framework of our method. The figure mainly contains fourth module: \textit{Image Encoder},\textit{Knowledge Encoder}, \textit{Transformer Decoder},\textit{Report Filter}. The details of \textit{Report Filter} can be found in Fig~\ref{fig:report_processor}. It can filter and clean original medical reports. \textit{Image Encoder} and \textit{Knowledge Encoder} are used to encoder the input of different modalities and \textit{Transformer Decoder} are used for cross-modality interaction. Contrastive loss and CE loss are adopted to calculate the final loss.}
    \label{fig:network}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{latex/figure/report_processor.pdf}
    \caption{The flowchart of the report filter module. A report is first filtered by a pre-trained filter. Then it is viewed as a set of triplets. The \textit{Location} part is embeded as a vector and mixed with some negative locations for contrastive loss and the \textit{``Exist''} part is used for CE loss.}
    \label{fig:report_processor}
\end{figure}
In this section we introduce our method generally.

First, we use a report text filter module $F_{text}$ which can re-modify the reports into a set of triplets. A triplet can be viewed as a set $\left\{[{\rm Observation}], [ {\rm Location}],[ {\rm Exist}]\right\}$. For instance, a triplet ${\{ [{\rm Opacity}], [ {\rm Right\ lower\ lobe}], [{\rm True}]\}}$ indicates there is opacity on the right lower lobe of a patient. Denote the original report as a set of sentences, ${\rm R}=\left \{s_1,s_2,...,s_i\right\}$, the the filter operation can be formulated as follow:
\begin{equation}
    F_{text} ({\rm R}) = \left\{  F_{text}({\rm s_1}), F_{text}({\rm s_2}), ..., F_{text} ({\rm s_i}) \right\},
\end{equation}
\begin{equation}
    F_{text} ({\rm s_i}) =\left\{[{\rm Observation_i}],[{\rm Location_i}],[{\rm Exist_i}]\right\}.
\end{equation}
More details about this will be discussed in the section~\ref{RepFil}.


With the triplets, we can re-modify the original retrieval question from the image-text level into image-entity level. In former works, the pre-train task is classically designed as asking the network whether a image matches a report, while in our flowchart the task is instead designed as asking the network whether an entity exist in a image and where it locates in. This is more fine-grained and can dismiss the impacts of noisy synonyms with different grammars. In the triplets, the $[{\rm Exist}]$ components can be naturally used as a binary classification label. For the $[{\rm Location}]$ component, we use a prompt \textit{``It is located at [location]''} with a pre-trained text encoder to get the embedding of the positive locations $f_{PL} \in R^{1\times D_1}$. With similar operation, we can randomly sample $M$ negative locations and get their embeddings $f_{NL} \in R^{M\times D_1}$ where $M$ is a hyper-parameter controls how many negative locations are sampled and $D_1$ is the embedding dim of the location features. With $f_{PL}$ and  $f_{NL}$ we can calculate contrastive loss to guide the network to distinguish the entity locations.

Our main framework is shown as Fig.~\ref{fig:network}. During training the input of the network is an image $I \in R^{H\times W \times C}$ and an entity list ${\rm E}$. ${\rm E}$ is a close entity set contains $N$ entities that mostly appear in the reports. The whole network is combined with an image encoder $E_{img}$, a knowledge encoder $E_{k}$, a transformer decoder $D_{trans}$ and two linear heads for Contrastive and CE loss separately. It can be denoted as a function $F_{net}$ formulated as
\begin{equation}
    F_{net}(I,E) = \left \{ f_{ex},f_{loc}\right\},
\end{equation}
where $f_{ex} \in R^{N \times 2}$ is the output of the CE head, representing the existence prediction of different entities and $f_{loc} \in R^{N \times D_1}$ is the output of the contrastive head, representing the location prediction of them. The final loss consists of two items. One is the mean BCE loss of different entities on existence
\begin{equation}
    \begin{split}
    L_{BCE} = -\frac{1}{N} \sum_{i=1}^{N}[\mathcal{I}([{\rm Exist_i}])\times log(\sigma(f_{ex}))\\ 
    + (1-\mathcal{I}([{\rm Exist_i}])\times log(1-\sigma(f_{ex})) ],
    \end{split}
\end{equation}


where $\mathcal{I}(\bullet)$ is an indicator functions. It equals one if the observation exists and zero otherwise. $\sigma(\bullet)$ represents the sigmoid function.

The other is the mean contrastive loss on locations
\begin{equation}
    \begin{split}
        L_{con} = -\frac{1}{N} \sum_{i=1}^{N}\frac{e^{<f_{loc},f_{PL}>/\gamma}}{\sum_{k=1}^{M}e^{<f_{loc},f_{NL_k}>/\gamma}},
    \end{split}
\end{equation}
where $<\bullet,\bullet>$ represent the inner Product of two vectors. $\gamma$ is a temperature hyper-parameter.


The final loss is the sum of the two
\begin{equation}
    L_{final} = L_{con} +L_{BCE}.
\end{equation}

For the sub-module $E_{img}$ in function $F_{net}$, We generally follow the classical ResNet50~\cite{he2016deep} structure to design the $E_{img}$ and reshape the final output into our desired shape. $E_{img}$ encodes the image and get the embedding of different image patches,
\begin{equation}
    E_{img}(I) = f_{img},
\end{equation}
where $f_{img} \in R^{P^2 \times D_2}$. $P^2$ represents the patch numbers after encoding and $D_2$ represents the embedding dim of the image.  Next, we will introduce the report filter $F_{text}$ and the other two sub-modules in function $F_{net}$, the knowledge encoder $E_k$ and the transformer decoder $D_{trans}$ in more details.

\subsection{Report Filter}
\label{RepFil}
Fist we talk about the report filter module. The key of this module is to filter out the image-specific knowledge from original reports with few information loss.

\textbf{Motivation.} Different from natural texts, which contain a lot of complex semantics,  semantics of medical reports are much more straightforward. The purpose of radiologists during writing reports is just to describe clearly whether abnormality exits, which disease the abnormality is and where the abnormality located at. Nevertheless, the grammar in the medical reports is complex and various, instead. For example, \textit{``No evidence of pneumothorax.''} and \textit{``There is no suspicious regions indicating pneumothorax.''} express the totally same facts while their grammar structures are quite different. Directly using the original report sentences to guide the network may cause the network struggle to capture the true meanings.


% \par{\noindent \bf Triplets Prompts with Report Filter. \hspace{3pt}} 

\textbf{Report Filter.} To handle the problem, we propose a report filter module to make the reports more structural, which is shown as Fig.~\ref{fig:report_processor}. Inspired by the success in medical NER, we use a pre-trained text filter~\cite{jain2021radgraph} to extract the most useful word entities in the reports, together with their relationships. Concretely, a report will be processed into a graph. The nodes are different entities and each entity has a label indicating whether it exists or not and is a medical observation or an anatomy location. There are relationship edges between different entities. A special relationship type is \textit{``located at''} indicating one entity located at the other.  We leverage this and regard the graph as triplets $\left\{[{\rm Observation}], [{\rm Location}],[{\rm Exist}]\right\}$, inspired by~\cite{yu2022anatomy}. There are some sentences that do not have any valid entities and they will be filtered out. We argue that this triplet format can not only get rid of complex syntax, but also remain the important information in reports, since it conclude the information that radiologists are most interested in. 

\subsection{Knowledge Encoder}
In this section, we mainly discuss about the knowledge encode $E_{k}$. The goal of this module is to learn prompt embeddings of different entities $f_{ent} \in R^{D_2}$ in set $E$ combining their medical expert-level knowledge. 

\textbf{Motivation.} The entities in $E$ are mainly some disease names, e.g. pneumonia and fracture. However, the disease names cannot reveal the relationship between different diseases. For instance, one of the vital imaging findings of pneumonia is the opacity appearance on the lung, which causes the entity \textit{``Pneumonia''} has strong correlation with the entity \textit{``Opacity''}. Besides, when dealing with new diseases, new diseases are often defined by various causes and symptoms. Using the name of the disease directly will cause the network completely fail to understand it, because the name does not provide any effective information.

\textbf{Knowledge Encoder.} To overcome this, we propose to take the description of different entities into consideration. For each entity, instead of name, we use the description of entity to expand the entity into a sentence. For example, entity \textit{``Pneumonia''} can be translated into \textit{``It is an condition of the lung primarily affecting the small air sacs known as alveolar. It may present with opacities and pleural effusion and it can increase the diagnostic accuracy of lung consolidation.''}. This description can reveal the definition and symptoms of each entity. Then we use a pre-trained text encoder $E_{text}$ with a flexible linear projection layer as our knowledge encoder $E_k$ to get the embedding of the entities, which can be denoted as
\begin{equation}
    E_k(Entity_{i}:Description_{i}) = f^i_e,
\end{equation}
where $f^i_e \in R^{D_2}$ represents the features of i-th entity and the embedding dim $D_2$ is same as the image features $f_{img}$.

Through adding the description knowledge, network can understand each entity, instead of just remembering their names. When handling a new entity, we just need to provide its description, the network can know what disease it is, assisting our network to handle unseen diseases.

\subsection{Transformer Decoder}
 Given the patch-level image features $f_{img}$ and the entity features $f_e$, we use a transformer decoder structure to get the location and existence prediction to each entity. Generally, we view the entity features $ f_{img} \in R^{N \times D_2}$ as transformer query input and  view image features $f_{img} \in R^{P^2 \times D_2}$ as transformer key and value input. The output of the transformer decoder can be denoted as $O_e \in R^{N \times D_2}$. The output is then go through a classification linear layer head and a contrastive linear layer head separately to get the final results $\left\{ f_{ex} , f_{loc}\right\}$. 
 
 In more detail, we adopt a parallel non-autoregressive Transformer decoder structure of multi layers~\cite{carion2020end}. In each decoder layer the queries are first passed through a self-attention layers and then followed by a multi-head attention layer between the modified queries and image features. In each head, the image features are processed by a linear key head and a linear value head as key embeddings and value embeddings independently. The value is weighted-added based on attention map, which is calculated by the soft-max dot product of the keys and queries.
 Finally, a feed-forward network gather the vector of different heads resulting in the output of this layer. The output vector of the former layer is considered as the entity query vector as the next layer. 
%  \xiaoman{I don't think the formulation is needed...}
%  In formulation, if denoting $l^{i}(\bullet,\bullet): R^{N \times D_2}\times R^{P^2\times D_2} \mapsto R^{N \times D_2}$ as the i-th layer, the procedure is expressed as:
%  \begin{equation}
%      l^{i}(r_{i-1},k_{img}) = r_i, r_0 = f_e.
%  \end{equation}
 
 \textbf{Discussion.} Different from the former classical methods~\cite{zhang2020contrastive} which calculate the alignment loss on the image level, the transformer decoder adopted here naturally can get the response on the patch level. Consequently, the image features $I_{img}$ will be more suitable for downstream segmentation tasks and the average of the attention map in each layers can be used directly for \textbf{zero-shot} grounding.
 
 
 
 
%\weidi{for t he existence of certain disease, we use binary cross-entropy, 
%with the existence label as groundtruth.}
% we use the triplets $\left\{[{\rm Entity}], [{\rm Location}],[{\rm Exist}]\right\}$ to calculate final loss. The $[{\rm Exist}]$ components can be naturally used as a binary classification label. BCE loss is adopted here as
% \begin{equation}
%     \begin{split}
%     \mathcal{L}_{\text{cls}} = -\frac{1}{E} \sum_{k=1}^{E}[\mathcal{I}([{\rm Exist_k}])\times log(\sigma(s^k))\\ 
%     + (1-\mathcal{I}([{\rm Exist_k}])\times log(1-\sigma(s^k)) ],
%     \end{split}
% \end{equation}

% where $\mathcal{I}(\bullet)$ is an indicator functions. It equals one if the entity exists and zero otherwise. $\sigma(\bullet)$ represents the sigmoid function.
%\weidi{too verbose, everyone knows what should be used for binary classification.}

%\weidi{I don't understand where the inferred spatial heatmap is applied to compute this loss, did you average pool the map ? or average pool the cross-attention map ?}






% \vspace{20pt}

% With the triplets, we can re-modify the original retrieval question from the image-text level into image-entity level. In former works, the pre-train task is classically designed as asking the network whether a image matches a report, while in our flowchart the task is instead designed as asking the network whether an entity exist in a image and where it locates in. This is more fine-grained and can dismiss the impacts of noisy synonyms with different grammars. In the triplets, the $[{\rm Exist}]$ components can be naturally used as a binary classification label. For the $[{\rm Location}]$ component, we use a prompt \textit{``It is located at [location]''} with a pre-trained text encoder to get the embedding of the positive locations $f_{PL} \in R^{1\times D_1}$. With similar operation, we can randomly sample $M$ negative locations and get their embeddings $f_{NL} \in R^{M\times D_1}$ where $M$ is a hyper-parameter controls how many negative locations are sampled and $D_1$ is the embedding dim of the location features. With $f_{PL}$ and  $f_{NL}$ we can calculate contrastive loss to guide the network to distinguish the entity locations.









% Our main framework is shown as Fig.~\ref{fig:network}. During training the input of the network is an image $I \in R^{H\times W \times C}$ and an entity list ${\rm E}$. ${\rm E}$ is a close entity set contains $N$ entities that mostly appear in the reports. The whole network is combined with an image encoder $E_{img}$, a knowledge encoder $E_{k}$, a transformer decoder $D_{trans}$ and two linear heads for Contrastive and CE loss separately. It can be denoted as a function $F_{net}$ formulated as
% \begin{equation}
%     F_{net}(I,E) = \left \{ f_{ex},f_{loc}\right\},
% \end{equation}
% where $f_{ex} \in R^{N \times 2}$ is the output of the CE head, representing the existence prediction of different entities and $f_{loc} \in R^{N \times D_1}$ is the output of the contrastive head, representing the location prediction of them. The final loss consists of two items. One is the mean BCE loss of different entities on existence
% \begin{equation}
%     \begin{split}
%     L_{BCE} = -\frac{1}{N} \sum_{i=1}^{N}[\mathcal{I}([{\rm Exist_i}])\times log(\sigma(f_{ex}))\\ 
%     + (1-\mathcal{I}([{\rm Exist_i}])\times log(1-\sigma(f_{ex})) ],
%     \end{split}
% \end{equation}


% where $\mathcal{I}(\bullet)$ is an indicator functions. It equals one if the observation exists and zero otherwise. $\sigma(\bullet)$ represents the sigmoid function.

% The other is the mean contrastive loss on locations
% \begin{equation}
%     \begin{split}
%         L_{con} = -\frac{1}{N} \sum_{i=1}^{N}\frac{e^{<f_{loc},f_{PL}>/\gamma}}{\sum_{k=1}^{M}e^{<f_{loc},f_{NL_k}>/\gamma}},
%     \end{split}
% \end{equation}
% where $<\bullet,\bullet>$ represent the inner Product of two vectors. $\gamma$ is a temperature hyper-parameter.


% The final loss is the sum of the two
% \begin{equation}
%     L_{final} = L_{con} +L_{BCE}.
% \end{equation}

% For the sub-module $E_{img}$ in function $F_{net}$, We generally follow the classical ResNet50~\cite{he2016deep} structure to design the $E_{img}$ and reshape the final output into our desired shape. $E_{img}$ encodes the image and get the embedding of different image patches,
% \begin{equation}
%     E_{img}(I) = f_{img},
% \end{equation}
% where $f_{img} \in R^{P^2 \times D_2}$. $P^2$ represents the patch numbers after encoding and $D_2$ represents the embedding dim of the image.  Next, we will introduce the report filter $F_{text}$ and the other two sub-modules in function $F_{net}$, the knowledge encoder $E_k$ and the transformer decoder $D_{trans}$ in more details.

% \subsection{Report Filter}
% \label{sec:preprocessing}


% First, we use a report text filter module $F_{text}$ which can re-modify the reports into a set of triplets. A triplet can be viewed as a set $\left\{[{\rm Observation}], [ {\rm Location}],[ {\rm Exist}]\right\}$. For instance, a triplet ${\{ [{\rm Opacity}], [ {\rm Right\ lower\ lobe}], [{\rm True}]\}}$ indicates there is opacity on the right lower lobe of a patient. Denote the original report as a set of sentences, ${\rm R}=\left \{s_1,s_2,...,s_i\right\}$, the the filter operation can be formulated as follow:
% \begin{equation}
%     F_{text} ({\rm R}) = \left\{  F_{text}({\rm s_1}), F_{text}({\rm s_2}), ..., F_{text} ({\rm s_i}) \right\},
% \end{equation}
% \begin{equation}
%     F_{text} ({\rm s_i}) =\left\{[{\rm Observation_i}],[{\rm Location_i}],[{\rm Exist_i}]\right\}.
% \end{equation}
% More details about this will be discussed in the section~\ref{RepFil}.

% Fist we talk about the report filter module. The key of this module is to filter out the image-specific knowledge from original reports with few information loss.

% \textbf{Motivation.} Different from natural texts, which contain a lot of complex semantics,  semantics of medical reports are much more straightforward. The purpose of radiologists during writing reports is just to describe clearly whether abnormality exits, which disease the abnormality is and where the abnormality located at. Nevertheless, the grammar in the medical reports is complex and various, instead. For example, \textit{``No evidence of pneumothorax.''} and \textit{``There is no suspicious regions indicating pneumothorax.''} express the totally same facts while their grammar structures are quite different. Directly using the original report sentences to guide the network may cause the network struggle to capture the true meanings.


% % \par{\noindent \bf Triplets Prompts with Report Filter. \hspace{3pt}} 

% \textbf{Report Filter.} To handle the problem, we propose a report filter module to make the reports more structural, which is shown as Fig.~\ref{fig:report_processor}. Inspired by the success in medical NER, we use a pre-trained text filter~\cite{jain2021radgraph} to extract the most useful word entities in the reports, together with their relationships. Concretely, a report will be processed into a graph. The nodes are different entities and each entity has a label indicating whether it exists or not and is a medical observation or an anatomy location. There are relationship edges between different entities. A special relationship type is \textit{``located at''} indicating one entity located at the other.  We leverage this and regard the graph as triplets $\left\{[{\rm Observation}], [{\rm Location}],[{\rm Exist}]\right\}$, inspired by~\cite{yu2022anatomy}. There are some sentences that do not have any valid entities and they will be filtered out. We argue that this triplet format can not only get rid of complex syntax, but also remain the important information in reports, since it conclude the information that radiologists are most interested in. 

% \subsection{Knowledge Encoder}
% \label{sec:knowledge}
% In this section, we mainly discuss about the knowledge encode $E_{k}$. The goal of this module is to learn prompt embeddings of different entities $f_{ent} \in R^{D_2}$ in set $E$ combining their medical expert-level knowledge. 

% \textbf{Motivation.} The entities in $E$ are mainly some disease names, e.g. pneumonia and fracture. However, the disease names cannot reveal the relationship between different diseases. For instance, one of the vital imaging findings of pneumonia is the opacity appearance on the lung, which causes the entity \textit{``Pneumonia''} has strong correlation with the entity \textit{``Opacity''}. Besides, when dealing with new diseases, new diseases are often defined by various causes and symptoms. Using the name of the disease directly will cause the network completely fail to understand it, because the name does not provide any effective information.

% \textbf{Knowledge Encoder.} To overcome this, we propose to take the description of different entities into consideration. For each entity, instead of name, we use the description of entity to expand the entity into a sentence. For example, entity \textit{``Pneumonia''} can be translated into \textit{``It is an condition of the lung primarily affecting the small air sacs known as alveolar. It may present with opacities and pleural effusion and it can increase the diagnostic accuracy of lung consolidation.''}. This description can reveal the definition and symptoms of each entity. Then we use a pre-trained text encoder $E_{text}$ with a flexible linear projection layer as our knowledge encoder $E_k$ to get the embedding of the entities, which can be denoted as
% \begin{equation}
%     E_k(Entity_{i}:Description_{i}) = f^i_e,
% \end{equation}
% where $f^i_e \in R^{D_2}$ represents the features of i-th entity and the embedding dim $D_2$ is same as the image features $f_{img}$.

% Through adding the description knowledge, network can understand each entity, instead of just remembering their names. When handling a new entity, we just need to provide its description, the network can know what disease it is, assisting our network to handle unseen diseases.

% \subsection{Transformer Decoder}
% \label{sec:architecture}
%  Given the patch-level image features $f_{img}$ and the entity features $f_e$, we use a transformer decoder structure to get the location and existence prediction to each entity. Generally, we view the entity features $ f_{img} \in R^{N \times D_2}$ as transformer query input and  view image features $f_{img} \in R^{P^2 \times D_2}$ as transformer key and value input. The output of the transformer decoder can be denoted as $O_e \in R^{N \times D_2}$. The output is then go through a classification linear layer head and a contrastive linear layer head separately to get the final results $\left\{ f_{ex} , f_{loc}\right\}$. 
 
%  In more detail, we adopt a parallel non-autoregressive Transformer decoder structure of multi layers~\cite{carion2020end}. In each decoder layer the queries are first passed through a self-attention layers and then followed by a multi-head attention layer between the modified queries and image features. In each head, the image features are processed by a linear key head and a linear value head as key embeddings and value embeddings independently. The value is weighted-added based on attention map, which is calculated by the soft-max dot product of the keys and queries.
%  Finally, a feed-forward network gather the vector of different heads resulting in the output of this layer. The output vector of the former layer is considered as the entity query vector as the next layer. 
% %  \xiaoman{I don't think the formulation is needed...}
% %  In formulation, if denoting $l^{i}(\bullet,\bullet): R^{N \times D_2}\times R^{P^2\times D_2} \mapsto R^{N \times D_2}$ as the i-th layer, the procedure is expressed as:
% %  \begin{equation}
% %      l^{i}(r_{i-1},k_{img}) = r_i, r_0 = f_e.
% %  \end{equation}
 
%  \textbf{Discussion.} Different from the former classical methods~\cite{zhang2020contrastive} which calculate the alignment loss on the image level, the transformer decoder adopted here naturally can get the response on the patch level. Consequently, the image features $I_{img}$ will be more suitable for downstream segmentation tasks and the average of the attention map in each layers can be used directly for \textbf{zero-shot} grounding.
 
 
 
